Graph Based Recommendations: From Data Representation to Feature Extraction and Application

Modeling users for the purpose of identifying their preferences and then personalizing services on the basis of these models is a complex task, primarily due to the need to take into consideration various explicit and implicit signals, missing or uncertain information, contextual aspects, and more. In this study, a novel generic approach for uncovering latent preference patterns from user data is proposed and evaluated. The approach relies on representing the data using graphs, and then systematically extracting graph-based features and using them to enrich the original user models. The extracted features encapsulate complex relationships between users, items, and metadata. The enhanced user models can then serve as an input to any recommendation algorithm. The proposed approach is domain-independent (demonstrated on data from movies, music, and business recommender systems), and is evaluated using several state-of-the-art machine learning methods, on different recommendation tasks, and using different evaluation metrics. The results show a unanimous improvement in the recommendation accuracy across tasks and domains. In addition, the evaluation provides a deeper analysis regarding the performance of the approach in special scenarios, including high sparsity and variability of ratings.

==> sec_case_studies.tex <==
The products of the presented approach are features that can be used to generate recommendations using existing machine-learning based recommendation methods. Those features can be used as standalone features (e.g., they suffice for generating highly accurate recommendations by themselves) or combined with existing features. Due to that, the baseline for comparison in the case studies is the performance of such methods, when used without the newly generated features.
In this section we present three case studies from different recommendation domains and how the graph based feature extraction approach contributes to improve recommendations accuracy in each one of them. The case studies demonstrate the approach on different recommendation tasks: predicting binary ratings, predicting a non binary rating value, and prediction of ranking based on an implicit interaction feedback metric (e.g., number of views/listens). We have evaluated the features on various machine-learning based recommendation methods, in order to see that their performance is consistent along them.
The machine-learning recommendation techniques that were used in the case studies are Random Forest \cite{breiman2001random} and Gradient Boosting \cite{friedman2001greedy}. Both are popular ensemble methods which have been used previously and shown to be among the best of their kind when winning recommendation \cite{koren2009bellkor} and general prediction \cite{yu2010feature} competitions. Those methods are also implemented in widely used machine-learning libraries \cite{pedregosa2011scikit,hall2009weka}. 
The metrics that we use to evaluate the accuracy of the recommendations are precision at K (P@K) \cite{ShaniG11} for the ranking and binary rating predictions, and RMSE for the star rating prediction. We compare the results to those of using existing features in the datasets or manually engineered ones.

We would like to note that comparing the results of the recommendation generation approach to other recommendation methods is outside the scope of this work and we refer the reader to general recommendation approaches comparisons done before \cite{jahrer2010combining,bellogin2013empirical,toscher2009bigchaos}, where it was demonstrated that ensemble methods (e.g., Random Forests) outperform standalone approaches such as Collaborative Filtering.

Case study 1 focused on the overall performance of the graph based approach, evaluating it on different domains and tasks. Case study 2 focused on how representing data using different graph schemes impacts recommendations. Last, case study 3 focused on how the graph based approach performs in border cases such as sparsity and variance in ratings.
The mapping between datasets and case studies is laid out in Table \ref{tab:dataset_to_casestudies_mapping}. Dataset \rom{3} could not have been used in Case Study \rom{2}, because it lacks the amount of entity and relationships types for that, while for Case Study \rom{3}, a single dataset has been chosen due to the experiment's complexity.
The next section provides characteristics of the datasets used, and afterwards we delve into the specific performance differences observed in each case, and across cases. 

\begin{table}
	\centering
	\caption{Mapping of Datasets to Case Studies}
	\begin{tabularx}{\textwidth}{p{0.17\textwidth}p{0.24\textwidth}p{0.24\textwidth}p{0.24\textwidth}}
		\toprule
		& Case Study \rom{1} - Overall performance& Case Study \rom{2} - Performance of different graph schemes & Case Study \rom{3} - Performance in cases of uncertainty\\
		\midrule
		Dataset \rom{1} - Last.FM& \checkmark & \checkmark & \\
		Dataset \rom{2} - Yelp& \checkmark & \checkmark & \checkmark\\
		Dataset \rom{3} - OSN& \checkmark &  & \\
		\bottomrule
	\end{tabularx}
	\label{tab:dataset_to_casestudies_mapping}
\end{table}

\subsection{Datasets}
\begin{table}[]
	\centering
	\caption{Summary of datasets characteristics}
	\begin{tabularx}{\textwidth}{p{0.2\textwidth}p{0.4\textwidth}p{0.4\textwidth}}
		\toprule[1pt]
		Dataset & Amount of Source and Target Entities & Graph Schemes \\
		\midrule[1pt]
		\rom{1} - Last.FM & 1,892 (users) \& 17,632 (artists) & Bipartite + Non-bipartite \\
		\midrule[0.5pt]
		\rom{2} - Yelp & 9,464 (users) \& 11,197 (businesses) & Bipartite + Bipartite with metadata \\
		\midrule[0.5pt]
		\rom{3} - OSN & 21,880 (users) \& 47,314 (interests) & Bipartite \\
		\bottomrule[1pt]
	\end{tabularx}
	\label{tab:dataset_summary}
\end{table}
Dataset \rom{1} - The first dataset is of users relevance feed provided to music artist via an online social network (Last.FM). The dataset is publicly available\footnote{http://grouplens.org/datasets/hetrec-2011/}, and was obtained by \cite{Cantador:RecSys2011}. The dataset consists of 1,892 users and 17,632 artists whom the users tagged and/or listened to. The amount of artists per users distribution is illustrated in Figure \ref{fig:items_per_users_across_datasets_cdfs} [left]. The dataset also contains social information regarding the social links established between Last.fm users (based on shared music interests online or real life friendship). There are overall 12,717 such bidirectional friendship links. There are in total 11,946 unique tags in the dataset, which were assigned by users to artists 186,479 times. Each user assigned on average 98.56 tags, 18.93 of them being distinct. Each artist was assigned 14.89 tags on average, with 8.76 of them being distinct. Additional characteristics of this dataset can be found at \cite{tiroshi2014graph}. Given the amount of relationships in the dataset (4 relationships -- \textit{[user, listens, artist]}, \textit{[user, uses, tag]}, \textit{[tag, used, artist]}, \textit{[user, friend, user]}) and \textit{[user, listens, artist}] chosen as the relationship to predict, the data can be represented via 8 graph schemes (based on the graph scheme generation process detailed in Algorithm \ref{algo:subset_graphs_generation} and Equation \ref{eq:relationship_combinations_simplified} for calculating the amount of generated graph schemes). Due to the recent interest in personalization in the social web \cite{brusilovsky2013preface}, we decided to focus our evaluation on graph schemes that incorporated social information and chose 4 out of 8 schemes. Those schemes are the ones that include  user-to-artist tagging and user-to-user friendships, and the schemes in which those were absent (for the purpose of comparison). The schemes are: 1. a bipartite graph that includes users and artist only (denoted as baseline, BL), 2. a non-bipartite graph that includes users, their social links, and artists (BL+F), 3. a non-bipartite graph that includes users, artists, and tags that were assigned by users to the artists (BL+T), and 4. a graph that includes all entities and relationships: users, tags, artists and social links (BL+T+F). The 4 graph schemes are illustrated in Figure \ref{fig:lastfm_graph_schemes}.
\begin{figure}[H]
	\centering
	\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{figures/lastfm_graph_schemes.png}
	\caption{Graph representation alternatives for dataset \rom{1}(Last.fm)}
	\label{fig:lastfm_graph_schemes}
\end{figure}

Dataset \rom{2} - The second dataset is of user relevance feedback given to businesses, such as: restaurants, shops, and services. The dataset was released by Yelp for the ACM Recommender Systems (RecSys) Conference 2013 challenge, and is publicly available\footnote{https://www.kaggle.com/c/yelp-recsys-2013/data}. For our analysis, we filtered out users with less than 5 reviews (representing $21\%$ of users, as illustrated in Figure \ref{fig:items_per_users_across_datasets_cdfs} [middle]), which results in 9,464 users providing 171,003 reviews, and the corresponding ratings, for 11,197 businesses. The average number of reviews per user is 18.07 (median=9) and the average number of reviews per business is 15.27 (median=5). A key observation regarding the dataset is the distribution of ratings which were almost all positive (more than 60\% of the ratings were at least 4 stars in a 5 stars scale), and with low variance across businesses and users, as illustrated in Figure \ref{fig:distribution_of_ratings_in_yelp}. This phenomenon is common in star ratings datasets, where users tend to review fewer items that they did not like \cite{ctfm_1}. We have filtered from the dataset user and business meta-data features that were highly sparse. Further analysis of the dataset and its properties is provided in \cite{tiroshi2014iui}. 

\begin{figure}[H]
	\centering
	\includegraphics[width=0.4\textwidth,height=\textheight,keepaspectratio]{figures/yelp_star_user_business_distribution_cdf.png}
	\caption{Distribution of ratings in dataset II (Yelp)}
	\label{fig:distribution_of_ratings_in_yelp}
\end{figure}

We modeled the dataset using two graph representations: a bipartite graph (user and business as vertices, connected with edges based on whether the user has reviewed the business) and a ‘tripartite’ graph (user, business, and meta-data vertices) non-directional graph. Those two models are illustrated in Figure \ref{fig:yelp_graph_schemes}. We extracted and populated a set of user and business related features and used these features to predict unknown user ratings for businesses. 

\begin{figure}[]
\begin{center}
  \includegraphics[width=0.6\textwidth]{figures/yelp_graph_schemes.png}
\end{center}
\caption{Graph representation alternatives for dataset \rom{2}(Yelp)}
\label{fig:yelp_graph_schemes}      
\end{figure}
 
Dataset \rom{3} - The last dataset is an Online Social Networking (OSN) profiles dataset that has been collected from 6 large networks: Facebook, LinkedIn, LastFM, Blogger, YouTube and LiveJournal. The profiles from those networks were linked and matched to each other based on whether they belong to the same user. This linkage was manually done by the users themselves, they mentioned their membership and corresponding user names on different online social networks. We extracted the lists of user interests, and categorized these into five domains: movies, music, books, TV, and general. The categorization was explicitly made by the users on Blogger, Facebook, and Youtube; all Lastfm interests were categorized as music; and no categorization was available on LinkedIn and LiveJournal, such that interests listed on these OSNs were treated as general. Users having one interest only in their aggregated profile, and interests having one user only associated with them, were removed from the dataset (as can be seen in Figure \ref{fig:items_per_users_across_datasets_cdfs} [right] that is a small fraction of the dataset). After these filterings, the dataset contains 21,880 users, with an average of 1.49 OSNs and 19.46 interests per user. Table \ref{tab:averageItem} shows the average amount of interests a user has on each network and domain combination. Additional characteristics of this dataset and details regarding how it was obtained can be found at \cite{chen2012wosn} and \cite{tiroshi2013cross}.

\begin{table}[]
	\centering
	\caption{Average number of interests per user in each domain and each network}
		\begin{tabularx}{\textwidth}{p{0.15\textwidth}p{0.15\textwidth}p{0.15\textwidth}p{0.15\textwidth}p{0.15\textwidth}p{0.15\textwidth}}
			~           & Uncategorized & Movies & Music & Books & TV \\
			\midrule[1pt]
			Blogger     & 5.913         & 2.976      & 4.676     & 2.577     & \textbf{--}   \\ 
			\midrule[0.5pt]
			Facebook  & 6.999         & 5.662      & 6.509      & 3.414     & 5.562  \\ \midrule[0.5pt]
			Lastfm      & \textbf{--}          & \textbf{--}       & 9.082      & \textbf{--}      & \textbf{--}   \\ 
			\midrule[0.5pt]
			LinkedIn    & 6.183         & \textbf{--}       & \textbf{--}       & \textbf{--}      & \textbf{--}   \\ 
			\midrule[0.5pt]
			LiveJournal & 20.69         & \textbf{--}      & \textbf{--}       & \textbf{--}      & \textbf{--}   \\ 
			\midrule[0.5pt]
			Youtube     & 1.288         & 1.278      & 1.395     & 1.177     & \textbf{--}   \\
			\bottomrule[1pt]
		\end{tabularx}
	\label{tab:averageItem} 
\end{table}

\begin{figure}[]
	\begin{center}
		\includegraphics[width=1.0\textwidth]{figures/items_per_users_across_datasets_cdfs_with_zoom.png}
	\end{center}
	\caption{Number of items per user distributions across datasets (X-axis number of items, Y-axis cumulative percentage in dataset). LastFM (left), Yelp (center) OSN (right). Both Yelp and the OSN datasets have few users with very few or a huge collection of items. While the Last.FM dataset has few users with few items and almost all users with an identical amount of items (50) due to the way the data was collected}
	\label{fig:items_per_users_across_datasets_cdfs}      
\end{figure}

\subsection{Case Studies}
\subsubsection{Case Study \rom{1} - Overall Performance of the Graph Based Approach}
\label{sec:case_study_1}
In this case study we are answering the broad question, \textit{How will graph features affect the performance of a recommender system in recommendation generation and feedback predictions in different domains and tasks?} Each of the datasets listed above, was represented by graphs, and graph based features were extracted from the graphs, using the approach detailed in section \ref{sec:graph_based_feature_extraction}. For each dataset, a recommendation task that matches it was defined. For the Yelp dataset of business ratings, the task defined was predicting which rating a user will provide to a selected business. The task defined for the Last.FM dataset was predicting to which artists users will listen the most. This task requires first to predict the amount of times each user will listen to each artist, and then ranking the artists in each user's evaluation set and choosing the top K artists and comparing to the validation set (each user's set of candidate artist was randomly chosen, and multiple sets sizes were evaluated). Last, for the OSN dataset, the task we defined was predicting which interest do users have in their profile.

The tasks were performed and evaluated in various scenarios: prediction with vs. without the graph features, prediction with users' related graph features vs. items' related graph features, and prediction using features of a minimal graph scheme (user-item bipartite graph) vs. extended graph schemes (such that contain metadata and features). 
All evaluations were conducted using cross validation \cite{kohavi1995study}, by splitting the original dataset into folds (5 folds in the Yelp and Last.FM datasets, and 10 in the OSN dataset). For each fold the complete graph representation was generated based on the entities from both training and test sets, excluding the relationships for prediction from the test set -- that is in order to prevent leakage of information from the test set to the graph metrics. The improvements reported below were all tested and found to be significant (t-test, p-value < 0.05).

For the first dataset (LastFM) the feature extraction process has shown to improve predictions of which artists will a user listen to by at least 48.21\% in precision. Four graph schemes were generated for the dataset (detailed in section \ref{sec:case_study_3}), and for each graph scheme the graph features listed in section \ref{sec:the_extracted_features} were extracted (`basic' graph features). In addition,  extended graph features were extracted from schemes that supported that (schemes with social data: BL+T, BL+F, BL+T+F in Figure \ref{fig:lastfm_graph_schemes}). The improvement was between the set of `basic' graph features extracted from a bipartite scheme (named BL for BaseLine) and scored 0.336 P@10, vs. the same set of graph features extracted from a graph scheme that included social tags nodes and links, and scored 0.498 P@10. A larger improvement, between 69\%-81\%, was noted when extended graph features were used. A combination of the extended graph features on a graph scheme that includes both social tags and friendships (BL+T and BL+F in Figure \ref{fig:lastfm_graph_schemes}) scored the highest P@10 equal to 0.571 (note: the extended features embed in them the basic features as described in the second case study).

Such improvements are also evident when experimenting with the second dataset (Yelp). Using features that are extracted from a graph based representations of the user-to-business data, the results show improvement in business ratings predictions when combined with basic and manually engineered features. The basic features are the unique identifiers of the users and businesses, and the manually engineered features consist of: number of reviews by user, average rating of a user, number of reviews for business, number of categories with which each business is associated with, average number of businesses in categories associated with the business, average rating of businesses in category, and location of the business. The largest improvement was of 5.9\% decrease in RMSE (decreasing the error by such percentage) between using the combination of graph features with basic and manually engineered ones (1.077 RMSE) vs. using only user-to-business pair associations (1.180 RMSE). A combination containing only the graph features also outperformed combinations containing only the manually engineered features (1.114 RMSE vs. 1.185 RMSE). This demonstrates the full benefits of the graph based approach, since extracting the graph features took less time than suggesting and creating the manual ones, and the graph features also out-performed the manual ones.

Last, in the third dataset of online social networks interest prediction, the graph-based features resulted in an improvement of binary predictions - whether a user will be interested in a subject or not. Using interest related graph based features (basic graph features) resulted in a precision of 9.8\% higher than using only user/interest IDs (precision of 0.56 vs. 0.51). Combining the graph features with manually engineered ones produced the highest precision 0.65 (among the manual engineered features are: whether an interest is listed on each of the social networks True/False, the amount of networks the interest appears on, whether the user is a member of each of the social networks True/False, and the amount of networks the user is a member of).

\begin{table}
	\centering
	\caption{Contribution of graph features across datasets}
	\begin{tabularx}{\textwidth}{p{0.07\textwidth}p{0.3\textwidth}p{0.1\textwidth}p{0.1\textwidth}p{0.3\textwidth}}
		\toprule[1pt]
		\parnoteclear
		Dataset & Task  & Metric & Learning Algorithm & Improvement\parnote{The differences in performance reported in this column have been tested statistically and found to be significant (p-value $<$ 0.05)}\\
		\midrule[1pt]
		\rom{1} & Rank artist based on predicted listens (regression)& Precision & Gradient Boost & 69\%-81\% improvement in precision between a bipartite scheme (0.336 P@10) vs. richer graph schemes (0.571 P@10)\\
		\midrule[0.5pt]
		\rom{2} & Predict star rating a user will give to a business (regression)& RMSE & Random Forests & 5.9\% decrease in RMSE between using all graph features (1.07 RMSE) vs. user-to-business associations (1.18 RMSE)\\
		\midrule[0.5pt]
		\rom{3} & Predict whether a user is interested in a subject or not (binary classification)& Precision & Random Forests  & 9.8\% improvement in precision when using interest related graph features (0.56)  vs. just the user-to-interest associations (0.51)\\
		\bottomrule[1pt]
	\end{tabularx}
	\parnotes
	\label{tab:addlabel}
\end{table}

In summary, the results of this case study show that when all the graph-based features have been used to complete each of the tasks, they resulted in improved recommendations across all datasets.

\subsubsection{Case Study \rom{2}: Different Graph Schemes and Their Impact On Results}
\label{sec:case_study_3}
As mentioned in the previous sections, various graph schemes can be generated for each dataset and each of them will produce different graph features values. The feature extraction process we have detailed takes into account all possible graph schemes and their corresponding generated features. Those features computed across different graphs scheme lead to the question - \textit{How the results of each scheme's features differ from one another?} In order to answer that we have represented two of the datasets, the Yelp and LastFM, using multiple schemes, and compared the results (the OSN dataset could not be used in this case study due to the low amount of entity types that result in a single graph representation). 

For the Yelp dataset with the task of business rating prediction, we compared between two graph schemes - a bipartite graph that contained only the users and businesses, and a second graph scheme - a bipartite graph that on top of user and business nodes also contained metadata nodes describing the businesses (the two graph schemes are illustrated in Figure \ref{fig:yelp_graph_schemes}, by the left and right graphs). The reason those were the only graph schemes created is that we have pre-filtered the dataset for sparse features -- features which had a very small amount of values relatively to the amount of rows. Such features would have resulted in most nodes of a group (e.g., users) being connected to a single node, which would render it meaningless. A set of graph features was generated for each scheme. Results showed that the simpler scheme, the one without business metadata, performed slightly better than the one with metadata (1\% RMSE difference, 1.11 RMSE of the bipartite graph vs. 1.13 for the bipartite with metadata graph). There were a few cases where the two feature sets performed differently on various data points, and thus the all features subset (which is a unification of the two schemes feature sets) performed better than the all except non-bipartite features, but not in a significant way. 

Our next evaluations on the impact of the graph schemes on performance were conducted on the Last.FM dataset. In this dataset we again evaluated a bipartite graph scheme (user nodes connected to artist nodes, BL in Figure \ref{fig:lastfm_graph_schemes}), but this time against three non-bipartite graphs. The first non-bipartite scheme was one that included social links between the users (Figure \ref{fig:lastfm_graph_schemes}, BL + F), the second was a scheme that included tag nodes connected both to the user and artist nodes based on whether they tagged/were tagged with the tag (Figure \ref{fig:lastfm_graph_schemes}, BL+T), and the third scheme included both tags and social links (Figure \ref{fig:lastfm_graph_schemes}, BL + T + F). As mentioned in the previous case study, two sets of graph features were extracted for each graph scheme, a set of basic graph features, and a set of extended graph features. The basic features set is shared across all schemes, and is composed of the features listed in Section \ref{sec:the_extracted_features}. The extended graph features set is composed of the basic features \textit{along with} features that were extracted based on the availability of social data in each scheme, the entities on which the extended features are based differ from one scheme to another\footnote{The process of extracting the extended features is automatic and detailed in Algorithm \ref{algo:feature_extraction} lines 13-20. The categorization of the features to ’basic’ and ’extended’ was manually done for the purpose of the evaluation.}. The general trend that was noticed in this experiment was that adding more types of entities to the graph improved the results. 

Figure \ref{fig:effect_of_social_link_features} shows the P@10 values averaged across all test set users, as obtained for the BL, BL+T, BL+F, and BL+T+F graph models, when using both the basic and extended graph features. The boundaries of the boxes denote the 25th and 75th percentile of P@10, and the average P@10 is marked by the dots inside the boxes.
First, we clearly observe that the inclusion of the social auxiliary data of either the artist tags or friendships links substantially improves P@10. When both the tags and friendship links are included in the BL+T+F model, we observe the highest average P@10. An improvement of 84\% with respect to the BL model that includes no auxiliary data is statistically significant. Noted is a modest improvement (9\%) of the BL+T+F model with respect to the best-performing model that included either the tag or the friendship data. This shows that including both types of social auxiliary data further improves the accuracy of the recommendations.

The BL+T and BL+F models obtain very similar P@10 scores, showing the positive effect of the inclusion of auxiliary data in the graph schemes. However, as noted in the dataset analysis, the tag data includes more than 186K user-artist tags, whereas the friendship data consists of only 12K user-to-user links. The observation that the obtained precision is similar indicates that a single user friendship link is more influential than a single artist tag and yields a greater improvement in the recommendation accuracy.

We note that out of the three graph models with the basic feature set, the lowest P@10 is achieved, somewhat surprisingly, by $F_{BL+T+F}$ (as can be seen in Figure \ref{fig:effect_on_graph_metrics} right most dotted boxplot). We conjecture that including both types of social data but not extracting and populating the new features leads to redundancy in the graph and degrades the performance of the recommender.

\begin{figure}
	\centering
	\includegraphics[width=0.3\textwidth,height=0.3\textwidth,keepaspectratio]{figures/lastfm_p@10.png}
	\caption{Average precision for the four graph schemes, when using all generated graph features -- basic and extended (on a candidate size of 150)}
	\label{fig:effect_of_social_link_features}
\end{figure}

We also evaluated how features which availability is dependent on the graph scheme would affect the results (e.g., `ratio\_of\_shared\_neighbors\_of\_type' with \textit{type} equal to \textit{tags}, which is equivalent to `ratio of shared tags' between a user and an artist, can only be computed on a graph that contains tags). In order to do that, an extended feature set is computed on each scheme that supports that (all schemes except BL). The extended feature set included the basic graph features, plus those two: `ratio\_of\_shared\_neighbors' (ratio between intersection of neighbors and their unification) and `ratio\_of\_shared\_neighbors\_of\_type' (same as previous feature only with a filter on the type of neighbors). Extended feature sets of the scheme with the tags and the scheme with the social links, both performed better than the basic graphs features of the bipartite graph (10\% and 12\% improvement respectively). This is illustrated in Figure \ref{fig:effect_on_graph_metrics}, the basic feature set is denoted as $F$ and the extended feature set as $\hat{F}$. The extended feature set of the scheme that had both the tags and social links performed the best, with a 29\% improvement relatively to the baseline. Also noticed was that the social links, even thought that in quantity they were fewer than the amount of tags (less data), the graph scheme that included them only performed better than the one that included only tags. We assume this is caused by social links indirectly linking users to more significant artist, than tags do (tags were less shared among users). In a dataset where tags are less shared among users, the tags tell us less about the global feedback of other users.

\begin{figure}
	\centering
	\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{figures/boxplots_bl_bl+delta_addon50.png}
	\caption{Precision of the extended (solid boxes) vs the basic (dotted boxes) feature sets for the four graph models}
	\label{fig:effect_on_graph_metrics}
\end{figure}





==> sec_case_study3.tex <==
\subsection{Case Study \rom{3}: Performance of the Graph-based Approach in Cases of High Variability and Sparsity}
\label{ch:evaluation3}
After establishing that features extracted from graph
representations contribute to the improvement in recommendation
and prediction accuracy, a deeper question that needs to be
answered is \textit{``How do graph features perform in different levels of user/item feedback variance and sparsity?''}. Another question is how the features will perform as compared to native features in those situations.
The first Yelp dataset is used for this analysis. As a reminder,
this dataset is represented using two bipartite graphs: one with
business metadata nodes and the other without the business
metadata. The types of features that are used in the evaluation
are: basic (the user and business unique identifiers); manually
engineered (number of reviews by user, average rating of user,
number of reviews for business, number of categories with which
each business is associated, average number of businesses in
categories associated with the business, average rating of
businesses in categories associated with the business, the main category of the business, average degree of all businesses associated with the business's main category, and location of the business); and graph features,
extracted using the presented approach.

\subsubsection{Variability of Ratings}
\label{sec:case_study_2_variability} In order to assess the
robustness of various groups of features to highly variable
ratings, the Yelp dataset of business ratings (Dataset \rom{2})
with the task of predicting which star rating a user will give to
a business is used. For the analysis, the STD of ratings per
business was computed and the businesses were sorted and then
split into buckets based on these values. The buckets were defined
to be of equal size (same number of businesses in each bucket)
leading the STD margins of each bucket to be determined by the
businesses in it. Then, for each feature combination and each
bucket of businesses, the RMSE between the predicted star
rating and ground truth rating in the dataset was computed.

\begin{figure}[ht!]
	\begin{center}
		\includegraphics[width=0.6\textwidth]{gfx/rmse_per_std_bin_summary_selected_new.pdf}
	\end{center}
	\caption[Yelp - business performance analysis in cases of variability]{RMSE per equal-sized buckets of
		businesses based on their ratings' STD}
	\label{fig:rmse_per_std_bin_summary_selected}
\end{figure}
\begin{sloppypar}
	The results of this analysis are summarized in Figure
	\ref{fig:rmse_per_std_bin_summary_selected}, where the x-axis
	represents the STD buckets, the left-most bucket having the
	lowest range of STD [0 - 0.548] and the right most bucket
	having the highest range of STD (1.389 - 2.828]\footnote{The brackets match the mathematical notation for defining intervals. Square brackets (``['' or ``]'') indicate that the value to the right/left is within the interval, while round brackets (``('' or ``)'') indicate that the value to the right/left is excluded from the interval, but values smaller/greater than it are within it (until the opposing limit is reached).}. The color of the cells correlate with the RMSE value: the lighter the color, the more accurate are the predictions. Only a subset of feature combinations that are interesting to the analysis was selected for this analysis prior to the training. The selected combinations and their individual performance, when computed
	across all users without buckets, are listed in Table
	\ref{tab:tbl_selected_feature_combinations_rmse}. The selected
	combinations reflect the performance difference between using graph only features (``Graph'') and manually engineered features
	(``Manual\_Eng\_Features''), basic features (user and business
	IDs) and the unification of both (``AllExcept\_Graph''). Two
	additional single features that were selected are the average
	rating of businesses and average rating given by users. These
	provide naive predictions that minimize RMSE and are
	interesting in the context of varying levels of STD. It can
	be seen that as the variance in ratings grows, their accuracy
	drops (RMSE rises).
\end{sloppypar}
\begin{table}[ht!]
	\centering
	\resizebox{0.6\columnwidth}{!}{
		\begin{tabular}{lllr}
			\toprule
			& Features combination & Features &      RMSE \\
			\midrule
			1 & All\_Features &Basic $\cup$ Manual $\cup$ Graph&  1.076667 \\
			2 & Graph & Bipartite $\cup$ Tripartite &  1.114891 \\
			3 & AllExcept\_Graph & Basic $\cup$ Manual&  1.117572 \\
			4 & User\_AVG\_Rating &  & 1.138437 \\
			5 & Business\_AVG\_Rating &  & 1.139135 \\
			\rowcolor{LightGray}
			6 & Basic &  & 1.180921 \\
			7 & Manual Engineered&  & 1.185396 \\
			\bottomrule
		\end{tabular}
	}
	\caption[Yelp - selected results for rating variability analysis]{The selected feature combinations
		used for analyzing performance in relation to ratings variability. The trend presented in
		Figure \ref{fig:rmse_per_std_bin_summary_selected}, that the Graph feature set and  AllExcept\_Graph feature set
		complement each other in different cases of ratings variability
		and lead All\_Features to perform the best, is confirmed by the aggregated performance results presented here.}
	\label{tab:tbl_selected_feature_combinations_rmse}%
\end{table}%

The experiment shows that the behavior of the graph features
differs, statistically significantly, from the behavior of the
basic and manually engineered features extracted from the original
rating data. While using the graph features achieved low accuracy
in the low STD buckets (the value of the combination's left
most bucket is higher than four other combinations in the bucket.
Row 2, column 1 versus rows 1,3,4,5 in the same column), the graph
features perform better in the high STD buckets. Features
such as average user/business rating that are part of the manual
features group performed worse (e.g., cell in row 2, right-most
column versus cells in rows 3-7, right-most column). The
``All\_Features'' combination, which is composed of the extended
and graph features, benefits from them both and across the board
achieves the highest overall accuracy. The difference in
performance in the high STD buckets between ``All\_Features''
and ``AllExcept\_Graph'' features clearly shows that the graph
features complement the non-graph features by allowing more accurate
predictions to be generated for businesses with highly variable
ratings.

In summary, in this case graph features were more robust when
predicting ratings for businesses with variable ratings.

\subsubsection{Sparsity of Ratings}
\label{sec:case_study_2_sparsity}
\begin{sloppypar}
	A similar analysis was conducted for cases with high sparsity of
	user ratings. The performance of the recommender when predicting
	ratings for users/businesses with a low number of training ratings was evaluated. Following a methodology similar to that used in the variability analysis above, users/businesses were split into equal-sized buckets. However, this time, the split was according to the number of ratings available. Figure
	\ref{fig:rmse_per_amount_of_reviews_for_users_bin_summary_selected} summarizes the RMSE values obtained for each feature
	combination and each bucket of users. The left side of the x-axis refers to buckets with a high sparsity (low number) of ratings and the right side to buckets with a low sparsity. Figure \ref{fig:rmse_per_amount_of_reviews_for_biz_bin_summary_selected} does the same but from a business perspective, binning businesses based on the amount of ratings they received.
\end{sloppypar}

\begin{figure}[ht!]
	\subfloat[Per users]{
		\includegraphics[width=0.495\textwidth]{gfx/rmse_per_amount_of_reviews_for_users_bin_summary_selected_new.pdf}
	\label{fig:rmse_per_amount_of_reviews_for_users_bin_summary_selected}
	}
	\subfloat[Per business]{
		\includegraphics[width=0.495\textwidth]{gfx/rmse_per_amount_of_reviews_for_biz_bin_summary_selected_new.pdf}
	\label{fig:rmse_per_amount_of_reviews_for_biz_bin_summary_selected}
	}
	\caption{RMSE per equal-sized buckets, based on the number of ratings}
\end{figure}

\begin{sloppypar}
In general, the performance of the recommender improves as more
ratings are available for a user/business, and this trend is
consistent across all the evaluated combinations of features.
Again, the contribution of the graph features can be clearly seen.
A comparison of the performance of the ``All\_Features'' and the
``AllExcept\_Graph'' combinations reveals that the graph features
perform significantly better than other non-graph based features for
the three sparsest buckets (columns 1-3) and equally as well for
the rest of the buckets. It is this differentiation in performance
that leads to the overall improvement in the recommendations. It
can also be noticed that the graph features outperform the individual feature ``user average'' across all buckets (row 2 versus. row 6). The graph features also outperform the individual feature ``business average'' across all buckets in user based analysis (Figure \ref{fig:rmse_per_amount_of_reviews_for_users_bin_summary_selected}, row 2 versus. row 5). In the business based analysis (Figure \ref{fig:rmse_per_amount_of_reviews_for_biz_bin_summary_selected}), the graph features outperform the ``business average'' feature in the left most bucket by a large margin (16\%, row 2 RMSE=1.3334 versus. row 5 RMSE=1.5984), while on the other buckets the business average performs better by a very small margin (average and median of 1\% difference). Overall it can be seen that the individual features perform poorly when there is a small amount of training data.
\end{sloppypar}

In conclusion, and answering the question introduced at the
beginning of the section \textit{`How do graph features perform in different levels of user/item feedback variance and sparsity?'}, it has been shown that graph features strengthen the predictability of ratings in cases of high variability, in
addition to strengthening the predictability in cases of data
sparsity and unavailability of sufficient training data. This is
an important finding, which indicates that graph features have the
potential to alleviate the cold-start problem of recommender
systems. 

==> sec_conclusions.tex <==
In this study, a new approach for improving recommendations was
presented and evaluated. Unlike most studies, which focused on
addressing the recommendation problem by making improvements to
the recommendation methods, the presented approach does so by
suggesting a different way to look at datasets. By re-representing
the datasets using graphs and extracting features from those
graphs, all in a systematic fashion. New features and
relationships that were not visible in the tabular form are
uncovered. In this manner, applying this approach may compliment
classical approaches and further enhance them.

The methodology, implementation, and analysis of the approach were
described in detail and the approach was evaluated from various
perspectives, i.e., overall performance versus sensitivity
analysis. The evaluation was performed on multiple datasets of
different characteristics and recommendation tasks. The datasets
belonged to four different recommender system domains (movies,
music, businesses, and personal interests), part of which included
metadata and part social aspects, i.e, social links and shared
tags. The tasks varied from binary link prediction to 5 star
rating prediction and also to prediction of ranking.
State-of-the-art classifiers and regressors were used to generate
the predictions and it was shown that the approach's positive
effect applies across such techniques.

Overall, the graph-based representation and features resulted in
the generation of more precise recommendations. The contributions
to certain scenarios of high variability and high sparsity were
also demonstrated. Finally, the variations in performance of
various graph schemes and the justification for systematically
extracting them, due to that, was established. The approach presented was
implemented in a library and is being provided as open source
software for the community to use and build on-top. Given such a
library, the cost of generating additional features that can
improve recommendations becomes relatively cheap, in terms of
computation time and effort. It can be adopted as a natural
``first attempt'' when given a dataset and recommendation task, or
as a complementary aid to enhance manual feature engineering.

The study suggested and demonstrated the potential to improve
recommendations by exploiting the benefits of links between
entities and characteristics of entities extracted from the graph
representation. This study lays the foundations for exploring
further how graph features can enhance recommender systems and
automatic feature engineering for recommendation systems in
general. This section describes several directions of exploration,
from partial representations of temporal datasets to utilizing more advanced
graph representations, such as weighted and directed graphs.

Laying the foundations for engineering new features from a dataset by representing it as a graph opens a wide space of possibilities to be mapped. Three aspects that were identified during this study as possible next interesting routes to explore in future works follow.

\emph{Temporal Aspects} - Given a dataset including dated actions that are not sparse, the time aspect can be used to build different graphs. Each graph will
represent a ``snapshot'' in time and will either contain or exclude a link based on whether it was available in the dataset at that time. The question is how such graphs will affect the values of features extracted from them and how the features will perform in their respective tasks.

\emph{Weighted and Labeled Graphs} - Several features in the dataset can be used to
populate edge labels when constructing the graph based representation.
The labels, once set, can be taken into consideration in
some of the graph features being extracted. One example would be
to calculate a weighted PageRank that will have jumps from a
vertex to its neighbors based on a skewed probability correlated to the weight on the edge that is linking to the neighbor. This could lead to further improvement in recommendations/predictions; however, it requires fine-tuning of initial weights on edges that do not naturally have such (e.g., the relationship edges in the Last.fm dataset).

\emph{Directed Graphs} - Similarly, in cases where the direction of edges is suspected to be crucial, the process can be extended to evaluate this by generating additional graph representations, with various combinations of edge directions. For
example, in one variation edges will be directed from the source
vertex to the target vertex, in another, in the opposite
direction, and in a third there will be no direction. This will
guarantee coverage in terms of the generated features relative to
direction, and the performance of the features in the various
scenarios could be evaluated.

The effects of these modifications on the scalability of the
approach can be handled using the previously suggested methods,
either by scaling the computations, e.g., computing the features
of each subgraph in a separate process, or using distributed graph
computation libraries, or identifying heuristics for pruning the
subgraphs/features space. 

==> sec_future_work.tex <==
Extracting new features from a dataset by representing it in a new format opens a wide space to be mapped. Two aspects that will be interesting to explore but are outside of the scope for this work are:

Temporal Aspects - Given a dataset with dated actions in it which are not sparse, the time aspect can be used to build different graphs. Each graph will either contain or miss a link based on whether it was available in the dataset at that time. The question is how will such graphs affect the values of features extracted from them? And how would those features perform in their respective tasks.

Weighted and Directed Graphs - 
Several features in the dataset can be used to populate edge labels when constructing the graph base representation. For example in the first dataset the amount of listens can be used as a label on the edges between users that links them to the artists they have listened to. On the second dataset the star rating a user has provided to a business can be used on the edge that links users to the businesses they have reviewed. Those labels, once set, can be taken into consideration in some of the graph features being extracted. One example would be to calculate a weighted PageRank that will have jumps from a vertex to its neighbors based on a skewed probability correlated to the weight on the edge that is linking to the neighbor. This could lead to farther improvement in recommendations/predictions however, requires fine-tuning of initial weights on edges that do not naturally have such (e.g., the relationship edges in the LastFM dataset).

Similarly, in cases which directness of edges is suspected to be crucial, the process can be extended to evaluate that by generating additional graph representations, with various combinations of edge directions. For example in one variation edges will be directed from the source node to the target node, in another they'll be in the opposite direction, and in a third there will not be a direction. This will grantee coverage in terms of the generated features relatively to directness, and the performance of the features in the various scenarios could be evaluated.

Finally, we are hoping to fully automate the SQL-to-Graph based representation phase in order to have a complete solution for the feature generation. This was out of the scope of this work since we first wanted to evaluate and generalize the graph features extraction process. A possible way to implement this would be to extract the entity relationship diagram from SQL database, use it as a graph scheme, and populate the graph with the entities instances.

